Search for the decays $X(3872)\to K_{S}^{0}K^{\pm}\pi^{\mp}$ and $K^*(892)\bar{K}$ at BESIII

Using a 10.9 fb$^{-1}$ data sample collected by the BESIII detector at center-of-mass energies from 4.16 to 4.34 GeV, we search for the charmless decays $X(3872) \to K_{S}^{0}K^{\pm}\pi^{\mp}$ and $K^*(892)\bar{K}$, where the $X(3872)$ is produced via the radiative process $e^+e^- \to \gamma X(3872)$. No significant signal is observed. We set upper limits on the relative branching fractions $\mathcal{B}[X(3872)\to K_S K^{\pm} \pi^{\mp}]/\mathcal{B}[X(3872)\to\pi^+\pi^- J/\psi] <0.07$ and $\mathcal{B}[X(3872)\to K^* (892)\bar{K}]/\mathcal{B}[X(3872)\to \pi^+\pi^- J/\psi] <0.10$ at the 90$\%$ confidence level. Additionally, upper limits on the product of the cross section $\sigma[e^+e^-\to\gamma X(3872)]$ and the branching fractions $\mathcal{B}[X(3872)\to K_{S}^{0}K^{\pm}\pi^{\mp}]$ and $\mathcal{B}[X(3872)\to K^*(892)\bar{K}]$ are reported at each energy point. In all cases, $K^*(892)\bar{K}$ refers to the sum of the modes $K^*(892)^+K^{-}+\text{c.c.}$ and $K^*(892)^0\bar{K}^0+\text{c.c.}$, where c.c. denotes the corresponding charge-conjugate modes.

==> authorlist_2025-08-14.tex <==
%% Saved at => 2025-08-14
M.~Ablikim$^{1}$\BESIIIorcid{0000-0002-3935-619X},
M.~N.~Achasov$^{4,c}$\BESIIIorcid{0000-0002-9400-8622},
P.~Adlarson$^{81}$\BESIIIorcid{0000-0001-6280-3851},
X.~C.~Ai$^{86}$\BESIIIorcid{0000-0003-3856-2415},
R.~Aliberti$^{39}$\BESIIIorcid{0000-0003-3500-4012},
A.~Amoroso$^{80A,80C}$\BESIIIorcid{0000-0002-3095-8610},
Q.~An$^{77,64,\dagger}$,
Y.~Bai$^{62}$\BESIIIorcid{0000-0001-6593-5665},
O.~Bakina$^{40}$\BESIIIorcid{0009-0005-0719-7461},
Y.~Ban$^{50,h}$\BESIIIorcid{0000-0002-1912-0374},
H.-R.~Bao$^{70}$\BESIIIorcid{0009-0002-7027-021X},
X.~L.~Bao$^{49}$\BESIIIorcid{0009-0000-3355-8359},
V.~Batozskaya$^{1,48}$\BESIIIorcid{0000-0003-1089-9200},
K.~Begzsuren$^{35}$,
N.~Berger$^{39}$\BESIIIorcid{0000-0002-9659-8507},
M.~Berlowski$^{48}$\BESIIIorcid{0000-0002-0080-6157},
M.~B.~Bertani$^{30A}$\BESIIIorcid{0000-0002-1836-502X},
D.~Bettoni$^{31A}$\BESIIIorcid{0000-0003-1042-8791},
F.~Bianchi$^{80A,80C}$\BESIIIorcid{0000-0002-1524-6236},
E.~Bianco$^{80A,80C}$,
A.~Bortone$^{80A,80C}$\BESIIIorcid{0000-0003-1577-5004},
I.~Boyko$^{40}$\BESIIIorcid{0000-0002-3355-4662},
R.~A.~Briere$^{5}$\BESIIIorcid{0000-0001-5229-1039},
A.~Brueggemann$^{74}$\BESIIIorcid{0009-0006-5224-894X},
H.~Cai$^{82}$\BESIIIorcid{0000-0003-0898-3673},
M.~H.~Cai$^{42,k,l}$\BESIIIorcid{0009-0004-2953-8629},
X.~Cai$^{1,64}$\BESIIIorcid{0000-0003-2244-0392},
A.~Calcaterra$^{30A}$\BESIIIorcid{0000-0003-2670-4826},
G.~F.~Cao$^{1,70}$\BESIIIorcid{0000-0003-3714-3665},
N.~Cao$^{1,70}$\BESIIIorcid{0000-0002-6540-217X},
S.~A.~Cetin$^{68A}$\BESIIIorcid{0000-0001-5050-8441},
X.~Y.~Chai$^{50,h}$\BESIIIorcid{0000-0003-1919-360X},
J.~F.~Chang$^{1,64}$\BESIIIorcid{0000-0003-3328-3214},
T.~T.~Chang$^{47}$\BESIIIorcid{0009-0000-8361-147X},
G.~R.~Che$^{47}$\BESIIIorcid{0000-0003-0158-2746},
Y.~Z.~Che$^{1,64,70}$\BESIIIorcid{0009-0008-4382-8736},
C.~H.~Chen$^{10}$\BESIIIorcid{0009-0008-8029-3240},
Chao~Chen$^{60}$\BESIIIorcid{0009-0000-3090-4148},
G.~Chen$^{1}$\BESIIIorcid{0000-0003-3058-0547},
H.~S.~Chen$^{1,70}$\BESIIIorcid{0000-0001-8672-8227},
H.~Y.~Chen$^{21}$\BESIIIorcid{0009-0009-2165-7910},
M.~L.~Chen$^{1,64,70}$\BESIIIorcid{0000-0002-2725-6036},
S.~J.~Chen$^{46}$\BESIIIorcid{0000-0003-0447-5348},
S.~M.~Chen$^{67}$\BESIIIorcid{0000-0002-2376-8413},
T.~Chen$^{1,70}$\BESIIIorcid{0009-0001-9273-6140},
W.~Chen$^{49}$\BESIIIorcid{0009-0002-6999-080X},
X.~R.~Chen$^{34,70}$\BESIIIorcid{0000-0001-8288-3983},
X.~T.~Chen$^{1,70}$\BESIIIorcid{0009-0003-3359-110X},
X.~Y.~Chen$^{12,g}$\BESIIIorcid{0009-0000-6210-1825},
Y.~B.~Chen$^{1,64}$\BESIIIorcid{0000-0001-9135-7723},
Y.~Q.~Chen$^{16}$\BESIIIorcid{0009-0008-0048-4849},
Z.~K.~Chen$^{65}$\BESIIIorcid{0009-0001-9690-0673},
J.~Cheng$^{49}$\BESIIIorcid{0000-0001-8250-770X},
L.~N.~Cheng$^{47}$\BESIIIorcid{0009-0003-1019-5294},
S.~K.~Choi$^{11}$\BESIIIorcid{0000-0003-2747-8277},
X.~Chu$^{12,g}$\BESIIIorcid{0009-0003-3025-1150},
G.~Cibinetto$^{31A}$\BESIIIorcid{0000-0002-3491-6231},
F.~Cossio$^{80C}$\BESIIIorcid{0000-0003-0454-3144},
J.~Cottee-Meldrum$^{69}$\BESIIIorcid{0009-0009-3900-6905},
H.~L.~Dai$^{1,64}$\BESIIIorcid{0000-0003-1770-3848},
J.~P.~Dai$^{84}$\BESIIIorcid{0000-0003-4802-4485},
X.~C.~Dai$^{67}$\BESIIIorcid{0000-0003-3395-7151},
A.~Dbeyssi$^{19}$,
R.~E.~de~Boer$^{3}$\BESIIIorcid{0000-0001-5846-2206},
D.~Dedovich$^{40}$\BESIIIorcid{0009-0009-1517-6504},
C.~Q.~Deng$^{78}$\BESIIIorcid{0009-0004-6810-2836},
Z.~Y.~Deng$^{1}$\BESIIIorcid{0000-0003-0440-3870},
A.~Denig$^{39}$\BESIIIorcid{0000-0001-7974-5854},
I.~Denisenko$^{40}$\BESIIIorcid{0000-0002-4408-1565},
M.~Destefanis$^{80A,80C}$\BESIIIorcid{0000-0003-1997-6751},
F.~De~Mori$^{80A,80C}$\BESIIIorcid{0000-0002-3951-272X},
X.~X.~Ding$^{50,h}$\BESIIIorcid{0009-0007-2024-4087},
Y.~Ding$^{44}$\BESIIIorcid{0009-0004-6383-6929},
Y.~X.~Ding$^{32}$\BESIIIorcid{0009-0000-9984-266X},
J.~Dong$^{1,64}$\BESIIIorcid{0000-0001-5761-0158},
L.~Y.~Dong$^{1,70}$\BESIIIorcid{0000-0002-4773-5050},
M.~Y.~Dong$^{1,64,70}$\BESIIIorcid{0000-0002-4359-3091},
X.~Dong$^{82}$\BESIIIorcid{0009-0004-3851-2674},
M.~C.~Du$^{1}$\BESIIIorcid{0000-0001-6975-2428},
S.~X.~Du$^{86}$\BESIIIorcid{0009-0002-4693-5429},
S.~X.~Du$^{12,g}$\BESIIIorcid{0009-0002-5682-0414},
X.~L.~Du$^{86}$\BESIIIorcid{0009-0004-4202-2539},
Y.~Y.~Duan$^{60}$\BESIIIorcid{0009-0004-2164-7089},
Z.~H.~Duan$^{46}$\BESIIIorcid{0009-0002-2501-9851},
P.~Egorov$^{40,b}$\BESIIIorcid{0009-0002-4804-3811},
G.~F.~Fan$^{46}$\BESIIIorcid{0009-0009-1445-4832},
J.~J.~Fan$^{20}$\BESIIIorcid{0009-0008-5248-9748},
Y.~H.~Fan$^{49}$\BESIIIorcid{0009-0009-4437-3742},
J.~Fang$^{1,64}$\BESIIIorcid{0000-0002-9906-296X},
J.~Fang$^{65}$\BESIIIorcid{0009-0007-1724-4764},
S.~S.~Fang$^{1,70}$\BESIIIorcid{0000-0001-5731-4113},
W.~X.~Fang$^{1}$\BESIIIorcid{0000-0002-5247-3833},
Y.~Q.~Fang$^{1,64,\dagger}$\BESIIIorcid{0000-0001-8630-6585},
L.~Fava$^{80B,80C}$\BESIIIorcid{0000-0002-3650-5778},
F.~Feldbauer$^{3}$\BESIIIorcid{0009-0002-4244-0541},
G.~Felici$^{30A}$\BESIIIorcid{0000-0001-8783-6115},
C.~Q.~Feng$^{77,64}$\BESIIIorcid{0000-0001-7859-7896},
J.~H.~Feng$^{16}$\BESIIIorcid{0009-0002-0732-4166},
L.~Feng$^{42,k,l}$\BESIIIorcid{0009-0005-1768-7755},
Q.~X.~Feng$^{42,k,l}$\BESIIIorcid{0009-0000-9769-0711},
Y.~T.~Feng$^{77,64}$\BESIIIorcid{0009-0003-6207-7804},
M.~Fritsch$^{3}$\BESIIIorcid{0000-0002-6463-8295},
C.~D.~Fu$^{1}$\BESIIIorcid{0000-0002-1155-6819},
J.~L.~Fu$^{70}$\BESIIIorcid{0000-0003-3177-2700},
Y.~W.~Fu$^{1,70}$\BESIIIorcid{0009-0004-4626-2505},
H.~Gao$^{70}$\BESIIIorcid{0000-0002-6025-6193},
Y.~Gao$^{77,64}$\BESIIIorcid{0000-0002-5047-4162},
Y.~N.~Gao$^{50,h}$\BESIIIorcid{0000-0003-1484-0943},
Y.~N.~Gao$^{20}$\BESIIIorcid{0009-0004-7033-0889},
Y.~Y.~Gao$^{32}$\BESIIIorcid{0009-0003-5977-9274},
Z.~Gao$^{47}$\BESIIIorcid{0009-0008-0493-0666},
S.~Garbolino$^{80C}$\BESIIIorcid{0000-0001-5604-1395},
I.~Garzia$^{31A,31B}$\BESIIIorcid{0000-0002-0412-4161},
L.~Ge$^{62}$\BESIIIorcid{0009-0001-6992-7328},
P.~T.~Ge$^{20}$\BESIIIorcid{0000-0001-7803-6351},
Z.~W.~Ge$^{46}$\BESIIIorcid{0009-0008-9170-0091},
C.~Geng$^{65}$\BESIIIorcid{0000-0001-6014-8419},
E.~M.~Gersabeck$^{73}$\BESIIIorcid{0000-0002-2860-6528},
A.~Gilman$^{75}$\BESIIIorcid{0000-0001-5934-7541},
K.~Goetzen$^{13}$\BESIIIorcid{0000-0002-0782-3806},
J.~D.~Gong$^{38}$\BESIIIorcid{0009-0003-1463-168X},
L.~Gong$^{44}$\BESIIIorcid{0000-0002-7265-3831},
W.~X.~Gong$^{1,64}$\BESIIIorcid{0000-0002-1557-4379},
W.~Gradl$^{39}$\BESIIIorcid{0000-0002-9974-8320},
S.~Gramigna$^{31A,31B}$\BESIIIorcid{0000-0001-9500-8192},
M.~Greco$^{80A,80C}$\BESIIIorcid{0000-0002-7299-7829},
M.~D.~Gu$^{55}$\BESIIIorcid{0009-0007-8773-366X},
M.~H.~Gu$^{1,64}$\BESIIIorcid{0000-0002-1823-9496},
C.~Y.~Guan$^{1,70}$\BESIIIorcid{0000-0002-7179-1298},
A.~Q.~Guo$^{34}$\BESIIIorcid{0000-0002-2430-7512},
J.~N.~Guo$^{12,g}$\BESIIIorcid{0009-0007-4905-2126},
L.~B.~Guo$^{45}$\BESIIIorcid{0000-0002-1282-5136},
M.~J.~Guo$^{54}$\BESIIIorcid{0009-0000-3374-1217},
R.~P.~Guo$^{53}$\BESIIIorcid{0000-0003-3785-2859},
X.~Guo$^{54}$\BESIIIorcid{0009-0002-2363-6880},
Y.~P.~Guo$^{12,g}$\BESIIIorcid{0000-0003-2185-9714},
A.~Guskov$^{40,b}$\BESIIIorcid{0000-0001-8532-1900},
J.~Gutierrez$^{29}$\BESIIIorcid{0009-0007-6774-6949},
T.~T.~Han$^{1}$\BESIIIorcid{0000-0001-6487-0281},
F.~Hanisch$^{3}$\BESIIIorcid{0009-0002-3770-1655},
K.~D.~Hao$^{77,64}$\BESIIIorcid{0009-0007-1855-9725},
X.~Q.~Hao$^{20}$\BESIIIorcid{0000-0003-1736-1235},
F.~A.~Harris$^{71}$\BESIIIorcid{0000-0002-0661-9301},
C.~Z.~He$^{50,h}$\BESIIIorcid{0009-0002-1500-3629},
K.~L.~He$^{1,70}$\BESIIIorcid{0000-0001-8930-4825},
F.~H.~Heinsius$^{3}$\BESIIIorcid{0000-0002-9545-5117},
C.~H.~Heinz$^{39}$\BESIIIorcid{0009-0008-2654-3034},
Y.~K.~Heng$^{1,64,70}$\BESIIIorcid{0000-0002-8483-690X},
C.~Herold$^{66}$\BESIIIorcid{0000-0002-0315-6823},
P.~C.~Hong$^{38}$\BESIIIorcid{0000-0003-4827-0301},
G.~Y.~Hou$^{1,70}$\BESIIIorcid{0009-0005-0413-3825},
X.~T.~Hou$^{1,70}$\BESIIIorcid{0009-0008-0470-2102},
Y.~R.~Hou$^{70}$\BESIIIorcid{0000-0001-6454-278X},
Z.~L.~Hou$^{1}$\BESIIIorcid{0000-0001-7144-2234},
H.~M.~Hu$^{1,70}$\BESIIIorcid{0000-0002-9958-379X},
J.~F.~Hu$^{61,j}$\BESIIIorcid{0000-0002-8227-4544},
Q.~P.~Hu$^{77,64}$\BESIIIorcid{0000-0002-9705-7518},
S.~L.~Hu$^{12,g}$\BESIIIorcid{0009-0009-4340-077X},
T.~Hu$^{1,64,70}$\BESIIIorcid{0000-0003-1620-983X},
Y.~Hu$^{1}$\BESIIIorcid{0000-0002-2033-381X},
Z.~M.~Hu$^{65}$\BESIIIorcid{0009-0008-4432-4492},
G.~S.~Huang$^{77,64}$\BESIIIorcid{0000-0002-7510-3181},
K.~X.~Huang$^{65}$\BESIIIorcid{0000-0003-4459-3234},
L.~Q.~Huang$^{34,70}$\BESIIIorcid{0000-0001-7517-6084},
P.~Huang$^{46}$\BESIIIorcid{0009-0004-5394-2541},
X.~T.~Huang$^{54}$\BESIIIorcid{0000-0002-9455-1967},
Y.~P.~Huang$^{1}$\BESIIIorcid{0000-0002-5972-2855},
Y.~S.~Huang$^{65}$\BESIIIorcid{0000-0001-5188-6719},
T.~Hussain$^{79}$\BESIIIorcid{0000-0002-5641-1787},
N.~H\"usken$^{39}$\BESIIIorcid{0000-0001-8971-9836},
N.~in~der~Wiesche$^{74}$\BESIIIorcid{0009-0007-2605-820X},
J.~Jackson$^{29}$\BESIIIorcid{0009-0009-0959-3045},
Q.~Ji$^{1}$\BESIIIorcid{0000-0003-4391-4390},
Q.~P.~Ji$^{20}$\BESIIIorcid{0000-0003-2963-2565},
W.~Ji$^{1,70}$\BESIIIorcid{0009-0004-5704-4431},
X.~B.~Ji$^{1,70}$\BESIIIorcid{0000-0002-6337-5040},
X.~L.~Ji$^{1,64}$\BESIIIorcid{0000-0002-1913-1997},
X.~Q.~Jia$^{54}$\BESIIIorcid{0009-0003-3348-2894},
Z.~K.~Jia$^{77,64}$\BESIIIorcid{0000-0002-4774-5961},
D.~Jiang$^{1,70}$\BESIIIorcid{0009-0009-1865-6650},
H.~B.~Jiang$^{82}$\BESIIIorcid{0000-0003-1415-6332},
P.~C.~Jiang$^{50,h}$\BESIIIorcid{0000-0002-4947-961X},
S.~J.~Jiang$^{10}$\BESIIIorcid{0009-0000-8448-1531},
X.~S.~Jiang$^{1,64,70}$\BESIIIorcid{0000-0001-5685-4249},
J.~B.~Jiao$^{54}$\BESIIIorcid{0000-0002-1940-7316},
J.~K.~Jiao$^{38}$\BESIIIorcid{0009-0003-3115-0837},
Z.~Jiao$^{25}$\BESIIIorcid{0009-0009-6288-7042},
L.~C.~L.~Jin$^{1}$\BESIIIorcid{0009-0003-4413-3729},
S.~Jin$^{46}$\BESIIIorcid{0000-0002-5076-7803},
Y.~Jin$^{72}$\BESIIIorcid{0000-0002-7067-8752},
M.~Q.~Jing$^{1,70}$\BESIIIorcid{0000-0003-3769-0431},
X.~M.~Jing$^{70}$\BESIIIorcid{0009-0000-2778-9978},
T.~Johansson$^{81}$\BESIIIorcid{0000-0002-6945-716X},
S.~Kabana$^{36}$\BESIIIorcid{0000-0003-0568-5750},
X.~L.~Kang$^{10}$\BESIIIorcid{0000-0001-7809-6389},
X.~S.~Kang$^{44}$\BESIIIorcid{0000-0001-7293-7116},
B.~C.~Ke$^{86}$\BESIIIorcid{0000-0003-0397-1315},
V.~Khachatryan$^{29}$\BESIIIorcid{0000-0003-2567-2930},
A.~Khoukaz$^{74}$\BESIIIorcid{0000-0001-7108-895X},
O.~B.~Kolcu$^{68A}$\BESIIIorcid{0000-0002-9177-1286},
B.~Kopf$^{3}$\BESIIIorcid{0000-0002-3103-2609},
L.~Kr\"oger$^{74}$\BESIIIorcid{0009-0001-1656-4877},
M.~Kuessner$^{3}$\BESIIIorcid{0000-0002-0028-0490},
X.~Kui$^{1,70}$\BESIIIorcid{0009-0005-4654-2088},
N.~Kumar$^{28}$\BESIIIorcid{0009-0004-7845-2768},
A.~Kupsc$^{48,81}$\BESIIIorcid{0000-0003-4937-2270},
W.~K\"uhn$^{41}$\BESIIIorcid{0000-0001-6018-9878},
Q.~Lan$^{78}$\BESIIIorcid{0009-0007-3215-4652},
W.~N.~Lan$^{20}$\BESIIIorcid{0000-0001-6607-772X},
T.~T.~Lei$^{77,64}$\BESIIIorcid{0009-0009-9880-7454},
M.~Lellmann$^{39}$\BESIIIorcid{0000-0002-2154-9292},
T.~Lenz$^{39}$\BESIIIorcid{0000-0001-9751-1971},
C.~Li$^{51}$\BESIIIorcid{0000-0002-5827-5774},
C.~Li$^{47}$\BESIIIorcid{0009-0005-8620-6118},
C.~H.~Li$^{45}$\BESIIIorcid{0000-0002-3240-4523},
C.~K.~Li$^{21}$\BESIIIorcid{0009-0006-8904-6014},
D.~M.~Li$^{86}$\BESIIIorcid{0000-0001-7632-3402},
F.~Li$^{1,64}$\BESIIIorcid{0000-0001-7427-0730},
G.~Li$^{1}$\BESIIIorcid{0000-0002-2207-8832},
H.~B.~Li$^{1,70}$\BESIIIorcid{0000-0002-6940-8093},
H.~J.~Li$^{20}$\BESIIIorcid{0000-0001-9275-4739},
H.~L.~Li$^{86}$\BESIIIorcid{0009-0005-3866-283X},
H.~N.~Li$^{61,j}$\BESIIIorcid{0000-0002-2366-9554},
Hui~Li$^{47}$\BESIIIorcid{0009-0006-4455-2562},
J.~R.~Li$^{67}$\BESIIIorcid{0000-0002-0181-7958},
J.~S.~Li$^{65}$\BESIIIorcid{0000-0003-1781-4863},
J.~W.~Li$^{54}$\BESIIIorcid{0000-0002-6158-6573},
K.~Li$^{1}$\BESIIIorcid{0000-0002-2545-0329},
K.~L.~Li$^{42,k,l}$\BESIIIorcid{0009-0007-2120-4845},
L.~J.~Li$^{1,70}$\BESIIIorcid{0009-0003-4636-9487},
Lei~Li$^{52}$\BESIIIorcid{0000-0001-8282-932X},
M.~H.~Li$^{47}$\BESIIIorcid{0009-0005-3701-8874},
M.~R.~Li$^{1,70}$\BESIIIorcid{0009-0001-6378-5410},
P.~L.~Li$^{70}$\BESIIIorcid{0000-0003-2740-9765},
P.~R.~Li$^{42,k,l}$\BESIIIorcid{0000-0002-1603-3646},
Q.~M.~Li$^{1,70}$\BESIIIorcid{0009-0004-9425-2678},
Q.~X.~Li$^{54}$\BESIIIorcid{0000-0002-8520-279X},
R.~Li$^{18,34}$\BESIIIorcid{0009-0000-2684-0751},
S.~X.~Li$^{12}$\BESIIIorcid{0000-0003-4669-1495},
Shanshan~Li$^{27,i}$\BESIIIorcid{0009-0008-1459-1282},
T.~Li$^{54}$\BESIIIorcid{0000-0002-4208-5167},
T.~Y.~Li$^{47}$\BESIIIorcid{0009-0004-2481-1163},
W.~D.~Li$^{1,70}$\BESIIIorcid{0000-0003-0633-4346},
W.~G.~Li$^{1,\dagger}$\BESIIIorcid{0000-0003-4836-712X},
X.~Li$^{1,70}$\BESIIIorcid{0009-0008-7455-3130},
X.~H.~Li$^{77,64}$\BESIIIorcid{0000-0002-1569-1495},
X.~K.~Li$^{50,h}$\BESIIIorcid{0009-0008-8476-3932},
X.~L.~Li$^{54}$\BESIIIorcid{0000-0002-5597-7375},
X.~Y.~Li$^{1,9}$\BESIIIorcid{0000-0003-2280-1119},
X.~Z.~Li$^{65}$\BESIIIorcid{0009-0008-4569-0857},
Y.~Li$^{20}$\BESIIIorcid{0009-0003-6785-3665},
Y.~G.~Li$^{70}$\BESIIIorcid{0000-0001-7922-256X},
Y.~P.~Li$^{38}$\BESIIIorcid{0009-0002-2401-9630},
Z.~H.~Li$^{42}$\BESIIIorcid{0009-0003-7638-4434},
Z.~J.~Li$^{65}$\BESIIIorcid{0000-0001-8377-8632},
Z.~X.~Li$^{47}$\BESIIIorcid{0009-0009-9684-362X},
Z.~Y.~Li$^{84}$\BESIIIorcid{0009-0003-6948-1762},
C.~Liang$^{46}$\BESIIIorcid{0009-0005-2251-7603},
H.~Liang$^{77,64}$\BESIIIorcid{0009-0004-9489-550X},
Y.~F.~Liang$^{59}$\BESIIIorcid{0009-0004-4540-8330},
Y.~T.~Liang$^{34,70}$\BESIIIorcid{0000-0003-3442-4701},
G.~R.~Liao$^{14}$\BESIIIorcid{0000-0003-1356-3614},
L.~B.~Liao$^{65}$\BESIIIorcid{0009-0006-4900-0695},
M.~H.~Liao$^{65}$\BESIIIorcid{0009-0007-2478-0768},
Y.~P.~Liao$^{1,70}$\BESIIIorcid{0009-0000-1981-0044},
J.~Libby$^{28}$\BESIIIorcid{0000-0002-1219-3247},
A.~Limphirat$^{66}$\BESIIIorcid{0000-0001-8915-0061},
D.~X.~Lin$^{34,70}$\BESIIIorcid{0000-0003-2943-9343},
L.~Q.~Lin$^{43}$\BESIIIorcid{0009-0008-9572-4074},
T.~Lin$^{1}$\BESIIIorcid{0000-0002-6450-9629},
B.~J.~Liu$^{1}$\BESIIIorcid{0000-0001-9664-5230},
B.~X.~Liu$^{82}$\BESIIIorcid{0009-0001-2423-1028},
C.~X.~Liu$^{1}$\BESIIIorcid{0000-0001-6781-148X},
F.~Liu$^{1}$\BESIIIorcid{0000-0002-8072-0926},
F.~H.~Liu$^{58}$\BESIIIorcid{0000-0002-2261-6899},
Feng~Liu$^{6}$\BESIIIorcid{0009-0000-0891-7495},
G.~M.~Liu$^{61,j}$\BESIIIorcid{0000-0001-5961-6588},
H.~Liu$^{42,k,l}$\BESIIIorcid{0000-0003-0271-2311},
H.~B.~Liu$^{15}$\BESIIIorcid{0000-0003-1695-3263},
H.~M.~Liu$^{1,70}$\BESIIIorcid{0000-0002-9975-2602},
Huihui~Liu$^{22}$\BESIIIorcid{0009-0006-4263-0803},
J.~B.~Liu$^{77,64}$\BESIIIorcid{0000-0003-3259-8775},
J.~J.~Liu$^{21}$\BESIIIorcid{0009-0007-4347-5347},
K.~Liu$^{42,k,l}$\BESIIIorcid{0000-0003-4529-3356},
K.~Liu$^{78}$\BESIIIorcid{0009-0002-5071-5437},
K.~Y.~Liu$^{44}$\BESIIIorcid{0000-0003-2126-3355},
Ke~Liu$^{23}$\BESIIIorcid{0000-0001-9812-4172},
L.~Liu$^{42}$\BESIIIorcid{0009-0004-0089-1410},
L.~C.~Liu$^{47}$\BESIIIorcid{0000-0003-1285-1534},
Lu~Liu$^{47}$\BESIIIorcid{0000-0002-6942-1095},
M.~H.~Liu$^{38}$\BESIIIorcid{0000-0002-9376-1487},
P.~L.~Liu$^{1}$\BESIIIorcid{0000-0002-9815-8898},
Q.~Liu$^{70}$\BESIIIorcid{0000-0003-4658-6361},
S.~B.~Liu$^{77,64}$\BESIIIorcid{0000-0002-4969-9508},
W.~M.~Liu$^{77,64}$\BESIIIorcid{0000-0002-1492-6037},
W.~T.~Liu$^{43}$\BESIIIorcid{0009-0006-0947-7667},
X.~Liu$^{42,k,l}$\BESIIIorcid{0000-0001-7481-4662},
X.~K.~Liu$^{42,k,l}$\BESIIIorcid{0009-0001-9001-5585},
X.~L.~Liu$^{12,g}$\BESIIIorcid{0000-0003-3946-9968},
X.~Y.~Liu$^{82}$\BESIIIorcid{0009-0009-8546-9935},
Y.~Liu$^{42,k,l}$\BESIIIorcid{0009-0002-0885-5145},
Y.~Liu$^{86}$\BESIIIorcid{0000-0002-3576-7004},
Y.~B.~Liu$^{47}$\BESIIIorcid{0009-0005-5206-3358},
Z.~A.~Liu$^{1,64,70}$\BESIIIorcid{0000-0002-2896-1386},
Z.~D.~Liu$^{10}$\BESIIIorcid{0009-0004-8155-4853},
Z.~Q.~Liu$^{54}$\BESIIIorcid{0000-0002-0290-3022},
Z.~Y.~Liu$^{42}$\BESIIIorcid{0009-0005-2139-5413},
X.~C.~Lou$^{1,64,70}$\BESIIIorcid{0000-0003-0867-2189},
H.~J.~Lu$^{25}$\BESIIIorcid{0009-0001-3763-7502},
J.~G.~Lu$^{1,64}$\BESIIIorcid{0000-0001-9566-5328},
X.~L.~Lu$^{16}$\BESIIIorcid{0009-0009-4532-4918},
Y.~Lu$^{7}$\BESIIIorcid{0000-0003-4416-6961},
Y.~H.~Lu$^{1,70}$\BESIIIorcid{0009-0004-5631-2203},
Y.~P.~Lu$^{1,64}$\BESIIIorcid{0000-0001-9070-5458},
Z.~H.~Lu$^{1,70}$\BESIIIorcid{0000-0001-6172-1707},
C.~L.~Luo$^{45}$\BESIIIorcid{0000-0001-5305-5572},
J.~R.~Luo$^{65}$\BESIIIorcid{0009-0006-0852-3027},
J.~S.~Luo$^{1,70}$\BESIIIorcid{0009-0003-3355-2661},
M.~X.~Luo$^{85}$,
T.~Luo$^{12,g}$\BESIIIorcid{0000-0001-5139-5784},
X.~L.~Luo$^{1,64}$\BESIIIorcid{0000-0003-2126-2862},
Z.~Y.~Lv$^{23}$\BESIIIorcid{0009-0002-1047-5053},
X.~R.~Lyu$^{70,o}$\BESIIIorcid{0000-0001-5689-9578},
Y.~F.~Lyu$^{47}$\BESIIIorcid{0000-0002-5653-9879},
Y.~H.~Lyu$^{86}$\BESIIIorcid{0009-0008-5792-6505},
F.~C.~Ma$^{44}$\BESIIIorcid{0000-0002-7080-0439},
H.~L.~Ma$^{1}$\BESIIIorcid{0000-0001-9771-2802},
Heng~Ma$^{27,i}$\BESIIIorcid{0009-0001-0655-6494},
J.~L.~Ma$^{1,70}$\BESIIIorcid{0009-0005-1351-3571},
L.~L.~Ma$^{54}$\BESIIIorcid{0000-0001-9717-1508},
L.~R.~Ma$^{72}$\BESIIIorcid{0009-0003-8455-9521},
Q.~M.~Ma$^{1}$\BESIIIorcid{0000-0002-3829-7044},
R.~Q.~Ma$^{1,70}$\BESIIIorcid{0000-0002-0852-3290},
R.~Y.~Ma$^{20}$\BESIIIorcid{0009-0000-9401-4478},
T.~Ma$^{77,64}$\BESIIIorcid{0009-0005-7739-2844},
X.~T.~Ma$^{1,70}$\BESIIIorcid{0000-0003-2636-9271},
X.~Y.~Ma$^{1,64}$\BESIIIorcid{0000-0001-9113-1476},
Y.~M.~Ma$^{34}$\BESIIIorcid{0000-0002-1640-3635},
F.~E.~Maas$^{19}$\BESIIIorcid{0000-0002-9271-1883},
I.~MacKay$^{75}$\BESIIIorcid{0000-0003-0171-7890},
M.~Maggiora$^{80A,80C}$\BESIIIorcid{0000-0003-4143-9127},
S.~Malde$^{75}$\BESIIIorcid{0000-0002-8179-0707},
Q.~A.~Malik$^{79}$\BESIIIorcid{0000-0002-2181-1940},
H.~X.~Mao$^{42,k,l}$\BESIIIorcid{0009-0001-9937-5368},
Y.~J.~Mao$^{50,h}$\BESIIIorcid{0009-0004-8518-3543},
Z.~P.~Mao$^{1}$\BESIIIorcid{0009-0000-3419-8412},
S.~Marcello$^{80A,80C}$\BESIIIorcid{0000-0003-4144-863X},
A.~Marshall$^{69}$\BESIIIorcid{0000-0002-9863-4954},
F.~M.~Melendi$^{31A,31B}$\BESIIIorcid{0009-0000-2378-1186},
Y.~H.~Meng$^{70}$\BESIIIorcid{0009-0004-6853-2078},
Z.~X.~Meng$^{72}$\BESIIIorcid{0000-0002-4462-7062},
G.~Mezzadri$^{31A}$\BESIIIorcid{0000-0003-0838-9631},
H.~Miao$^{1,70}$\BESIIIorcid{0000-0002-1936-5400},
T.~J.~Min$^{46}$\BESIIIorcid{0000-0003-2016-4849},
R.~E.~Mitchell$^{29}$\BESIIIorcid{0000-0003-2248-4109},
X.~H.~Mo$^{1,64,70}$\BESIIIorcid{0000-0003-2543-7236},
B.~Moses$^{29}$\BESIIIorcid{0009-0000-0942-8124},
N.~Yu.~Muchnoi$^{4,c}$\BESIIIorcid{0000-0003-2936-0029},
J.~Muskalla$^{39}$\BESIIIorcid{0009-0001-5006-370X},
Y.~Nefedov$^{40}$\BESIIIorcid{0000-0001-6168-5195},
F.~Nerling$^{19,e}$\BESIIIorcid{0000-0003-3581-7881},
H.~Neuwirth$^{74}$\BESIIIorcid{0009-0007-9628-0930},
Z.~Ning$^{1,64}$\BESIIIorcid{0000-0002-4884-5251},
S.~Nisar$^{33,a}$,
Q.~L.~Niu$^{42,k,l}$\BESIIIorcid{0009-0004-3290-2444},
W.~D.~Niu$^{12,g}$\BESIIIorcid{0009-0002-4360-3701},
Y.~Niu$^{54}$\BESIIIorcid{0009-0002-0611-2954},
C.~Normand$^{69}$\BESIIIorcid{0000-0001-5055-7710},
S.~L.~Olsen$^{11,70}$\BESIIIorcid{0000-0002-6388-9885},
Q.~Ouyang$^{1,64,70}$\BESIIIorcid{0000-0002-8186-0082},
S.~Pacetti$^{30B,30C}$\BESIIIorcid{0000-0002-6385-3508},
X.~Pan$^{60}$\BESIIIorcid{0000-0002-0423-8986},
Y.~Pan$^{62}$\BESIIIorcid{0009-0004-5760-1728},
A.~Pathak$^{11}$\BESIIIorcid{0000-0002-3185-5963},
Y.~P.~Pei$^{77,64}$\BESIIIorcid{0009-0009-4782-2611},
M.~Pelizaeus$^{3}$\BESIIIorcid{0009-0003-8021-7997},
H.~P.~Peng$^{77,64}$\BESIIIorcid{0000-0002-3461-0945},
X.~J.~Peng$^{42,k,l}$\BESIIIorcid{0009-0005-0889-8585},
Y.~Y.~Peng$^{42,k,l}$\BESIIIorcid{0009-0006-9266-4833},
K.~Peters$^{13,e}$\BESIIIorcid{0000-0001-7133-0662},
K.~Petridis$^{69}$\BESIIIorcid{0000-0001-7871-5119},
J.~L.~Ping$^{45}$\BESIIIorcid{0000-0002-6120-9962},
R.~G.~Ping$^{1,70}$\BESIIIorcid{0000-0002-9577-4855},
S.~Plura$^{39}$\BESIIIorcid{0000-0002-2048-7405},
V.~Prasad$^{38}$\BESIIIorcid{0000-0001-7395-2318},
F.~Z.~Qi$^{1}$\BESIIIorcid{0000-0002-0448-2620},
H.~R.~Qi$^{67}$\BESIIIorcid{0000-0002-9325-2308},
M.~Qi$^{46}$\BESIIIorcid{0000-0002-9221-0683},
S.~Qian$^{1,64}$\BESIIIorcid{0000-0002-2683-9117},
W.~B.~Qian$^{70}$\BESIIIorcid{0000-0003-3932-7556},
C.~F.~Qiao$^{70}$\BESIIIorcid{0000-0002-9174-7307},
J.~H.~Qiao$^{20}$\BESIIIorcid{0009-0000-1724-961X},
J.~J.~Qin$^{78}$\BESIIIorcid{0009-0002-5613-4262},
J.~L.~Qin$^{60}$\BESIIIorcid{0009-0005-8119-711X},
L.~Q.~Qin$^{14}$\BESIIIorcid{0000-0002-0195-3802},
L.~Y.~Qin$^{77,64}$\BESIIIorcid{0009-0000-6452-571X},
P.~B.~Qin$^{78}$\BESIIIorcid{0009-0009-5078-1021},
X.~P.~Qin$^{43}$\BESIIIorcid{0000-0001-7584-4046},
X.~S.~Qin$^{54}$\BESIIIorcid{0000-0002-5357-2294},
Z.~H.~Qin$^{1,64}$\BESIIIorcid{0000-0001-7946-5879},
J.~F.~Qiu$^{1}$\BESIIIorcid{0000-0002-3395-9555},
Z.~H.~Qu$^{78}$\BESIIIorcid{0009-0006-4695-4856},
J.~Rademacker$^{69}$\BESIIIorcid{0000-0003-2599-7209},
C.~F.~Redmer$^{39}$\BESIIIorcid{0000-0002-0845-1290},
A.~Rivetti$^{80C}$\BESIIIorcid{0000-0002-2628-5222},
M.~Rolo$^{80C}$\BESIIIorcid{0000-0001-8518-3755},
G.~Rong$^{1,70}$\BESIIIorcid{0000-0003-0363-0385},
S.~S.~Rong$^{1,70}$\BESIIIorcid{0009-0005-8952-0858},
F.~Rosini$^{30B,30C}$\BESIIIorcid{0009-0009-0080-9997},
Ch.~Rosner$^{19}$\BESIIIorcid{0000-0002-2301-2114},
M.~Q.~Ruan$^{1,64}$\BESIIIorcid{0000-0001-7553-9236},
N.~Salone$^{48,p}$\BESIIIorcid{0000-0003-2365-8916},
A.~Sarantsev$^{40,d}$\BESIIIorcid{0000-0001-8072-4276},
Y.~Schelhaas$^{39}$\BESIIIorcid{0009-0003-7259-1620},
K.~Schoenning$^{81}$\BESIIIorcid{0000-0002-3490-9584},
M.~Scodeggio$^{31A}$\BESIIIorcid{0000-0003-2064-050X},
W.~Shan$^{26}$\BESIIIorcid{0000-0003-2811-2218},
X.~Y.~Shan$^{77,64}$\BESIIIorcid{0000-0003-3176-4874},
Z.~J.~Shang$^{42,k,l}$\BESIIIorcid{0000-0002-5819-128X},
J.~F.~Shangguan$^{17}$\BESIIIorcid{0000-0002-0785-1399},
L.~G.~Shao$^{1,70}$\BESIIIorcid{0009-0007-9950-8443},
M.~Shao$^{77,64}$\BESIIIorcid{0000-0002-2268-5624},
C.~P.~Shen$^{12,g}$\BESIIIorcid{0000-0002-9012-4618},
H.~F.~Shen$^{1,9}$\BESIIIorcid{0009-0009-4406-1802},
W.~H.~Shen$^{70}$\BESIIIorcid{0009-0001-7101-8772},
X.~Y.~Shen$^{1,70}$\BESIIIorcid{0000-0002-6087-5517},
B.~A.~Shi$^{70}$\BESIIIorcid{0000-0002-5781-8933},
H.~Shi$^{77,64}$\BESIIIorcid{0009-0005-1170-1464},
J.~L.~Shi$^{8,q}$\BESIIIorcid{0009-0000-6832-523X},
J.~Y.~Shi$^{1}$\BESIIIorcid{0000-0002-8890-9934},
S.~Y.~Shi$^{78}$\BESIIIorcid{0009-0000-5735-8247},
X.~Shi$^{1,64}$\BESIIIorcid{0000-0001-9910-9345},
H.~L.~Song$^{77,64}$\BESIIIorcid{0009-0001-6303-7973},
J.~J.~Song$^{20}$\BESIIIorcid{0000-0002-9936-2241},
M.~H.~Song$^{42}$\BESIIIorcid{0009-0003-3762-4722},
T.~Z.~Song$^{65}$\BESIIIorcid{0009-0009-6536-5573},
W.~M.~Song$^{38}$\BESIIIorcid{0000-0003-1376-2293},
Y.~X.~Song$^{50,h,m}$\BESIIIorcid{0000-0003-0256-4320},
Zirong~Song$^{27,i}$\BESIIIorcid{0009-0001-4016-040X},
S.~Sosio$^{80A,80C}$\BESIIIorcid{0009-0008-0883-2334},
S.~Spataro$^{80A,80C}$\BESIIIorcid{0000-0001-9601-405X},
S.~Stansilaus$^{75}$\BESIIIorcid{0000-0003-1776-0498},
F.~Stieler$^{39}$\BESIIIorcid{0009-0003-9301-4005},
S.~S~Su$^{44}$\BESIIIorcid{0009-0002-3964-1756},
G.~B.~Sun$^{82}$\BESIIIorcid{0009-0008-6654-0858},
G.~X.~Sun$^{1}$\BESIIIorcid{0000-0003-4771-3000},
H.~Sun$^{70}$\BESIIIorcid{0009-0002-9774-3814},
H.~K.~Sun$^{1}$\BESIIIorcid{0000-0002-7850-9574},
J.~F.~Sun$^{20}$\BESIIIorcid{0000-0003-4742-4292},
K.~Sun$^{67}$\BESIIIorcid{0009-0004-3493-2567},
L.~Sun$^{82}$\BESIIIorcid{0000-0002-0034-2567},
R.~Sun$^{77}$\BESIIIorcid{0009-0009-3641-0398},
S.~S.~Sun$^{1,70}$\BESIIIorcid{0000-0002-0453-7388},
T.~Sun$^{56,f}$\BESIIIorcid{0000-0002-1602-1944},
W.~Y.~Sun$^{55}$\BESIIIorcid{0000-0001-5807-6874},
Y.~C.~Sun$^{82}$\BESIIIorcid{0009-0009-8756-8718},
Y.~H.~Sun$^{32}$\BESIIIorcid{0009-0007-6070-0876},
Y.~J.~Sun$^{77,64}$\BESIIIorcid{0000-0002-0249-5989},
Y.~Z.~Sun$^{1}$\BESIIIorcid{0000-0002-8505-1151},
Z.~Q.~Sun$^{1,70}$\BESIIIorcid{0009-0004-4660-1175},
Z.~T.~Sun$^{54}$\BESIIIorcid{0000-0002-8270-8146},
C.~J.~Tang$^{59}$,
G.~Y.~Tang$^{1}$\BESIIIorcid{0000-0003-3616-1642},
J.~Tang$^{65}$\BESIIIorcid{0000-0002-2926-2560},
J.~J.~Tang$^{77,64}$\BESIIIorcid{0009-0008-8708-015X},
L.~F.~Tang$^{43}$\BESIIIorcid{0009-0007-6829-1253},
Y.~A.~Tang$^{82}$\BESIIIorcid{0000-0002-6558-6730},
L.~Y.~Tao$^{78}$\BESIIIorcid{0009-0001-2631-7167},
M.~Tat$^{75}$\BESIIIorcid{0000-0002-6866-7085},
J.~X.~Teng$^{77,64}$\BESIIIorcid{0009-0001-2424-6019},
J.~Y.~Tian$^{77,64}$\BESIIIorcid{0009-0008-1298-3661},
W.~H.~Tian$^{65}$\BESIIIorcid{0000-0002-2379-104X},
Y.~Tian$^{34}$\BESIIIorcid{0009-0008-6030-4264},
Z.~F.~Tian$^{82}$\BESIIIorcid{0009-0005-6874-4641},
I.~Uman$^{68B}$\BESIIIorcid{0000-0003-4722-0097},
B.~Wang$^{1}$\BESIIIorcid{0000-0002-3581-1263},
B.~Wang$^{65}$\BESIIIorcid{0009-0004-9986-354X},
Bo~Wang$^{77,64}$\BESIIIorcid{0009-0002-6995-6476},
C.~Wang$^{42,k,l}$\BESIIIorcid{0009-0005-7413-441X},
C.~Wang$^{20}$\BESIIIorcid{0009-0001-6130-541X},
Cong~Wang$^{23}$\BESIIIorcid{0009-0006-4543-5843},
D.~Y.~Wang$^{50,h}$\BESIIIorcid{0000-0002-9013-1199},
H.~J.~Wang$^{42,k,l}$\BESIIIorcid{0009-0008-3130-0600},
H.~R.~Wang$^{83}$\BESIIIorcid{0009-0007-6297-7801},
J.~Wang$^{10}$\BESIIIorcid{0009-0004-9986-2483},
J.~J.~Wang$^{82}$\BESIIIorcid{0009-0006-7593-3739},
J.~P.~Wang$^{37}$\BESIIIorcid{0009-0004-8987-2004},
K.~Wang$^{1,64}$\BESIIIorcid{0000-0003-0548-6292},
L.~L.~Wang$^{1}$\BESIIIorcid{0000-0002-1476-6942},
L.~W.~Wang$^{38}$\BESIIIorcid{0009-0006-2932-1037},
M.~Wang$^{54}$\BESIIIorcid{0000-0003-4067-1127},
M.~Wang$^{77,64}$\BESIIIorcid{0009-0004-1473-3691},
N.~Y.~Wang$^{70}$\BESIIIorcid{0000-0002-6915-6607},
S.~Wang$^{42,k,l}$\BESIIIorcid{0000-0003-4624-0117},
Shun~Wang$^{63}$\BESIIIorcid{0000-0001-7683-101X},
T.~Wang$^{12,g}$\BESIIIorcid{0009-0009-5598-6157},
T.~J.~Wang$^{47}$\BESIIIorcid{0009-0003-2227-319X},
W.~Wang$^{65}$\BESIIIorcid{0000-0002-4728-6291},
W.~P.~Wang$^{39}$\BESIIIorcid{0000-0001-8479-8563},
X.~Wang$^{50,h}$\BESIIIorcid{0009-0005-4220-4364},
X.~F.~Wang$^{42,k,l}$\BESIIIorcid{0000-0001-8612-8045},
X.~L.~Wang$^{12,g}$\BESIIIorcid{0000-0001-5805-1255},
X.~N.~Wang$^{1,70}$\BESIIIorcid{0009-0009-6121-3396},
Xin~Wang$^{27,i}$\BESIIIorcid{0009-0004-0203-6055},
Y.~Wang$^{1}$\BESIIIorcid{0009-0003-2251-239X},
Y.~D.~Wang$^{49}$\BESIIIorcid{0000-0002-9907-133X},
Y.~F.~Wang$^{1,9,70}$\BESIIIorcid{0000-0001-8331-6980},
Y.~H.~Wang$^{42,k,l}$\BESIIIorcid{0000-0003-1988-4443},
Y.~J.~Wang$^{77,64}$\BESIIIorcid{0009-0007-6868-2588},
Y.~L.~Wang$^{20}$\BESIIIorcid{0000-0003-3979-4330},
Y.~N.~Wang$^{49}$\BESIIIorcid{0009-0000-6235-5526},
Y.~N.~Wang$^{82}$\BESIIIorcid{0009-0006-5473-9574},
Yaqian~Wang$^{18}$\BESIIIorcid{0000-0001-5060-1347},
Yi~Wang$^{67}$\BESIIIorcid{0009-0004-0665-5945},
Yuan~Wang$^{18,34}$\BESIIIorcid{0009-0004-7290-3169},
Z.~Wang$^{1,64}$\BESIIIorcid{0000-0001-5802-6949},
Z.~Wang$^{47}$\BESIIIorcid{0009-0008-9923-0725},
Z.~L.~Wang$^{2}$\BESIIIorcid{0009-0002-1524-043X},
Z.~Q.~Wang$^{12,g}$\BESIIIorcid{0009-0002-8685-595X},
Z.~Y.~Wang$^{1,70}$\BESIIIorcid{0000-0002-0245-3260},
Ziyi~Wang$^{70}$\BESIIIorcid{0000-0003-4410-6889},
D.~Wei$^{47}$\BESIIIorcid{0009-0002-1740-9024},
D.~H.~Wei$^{14}$\BESIIIorcid{0009-0003-7746-6909},
H.~R.~Wei$^{47}$\BESIIIorcid{0009-0006-8774-1574},
F.~Weidner$^{74}$\BESIIIorcid{0009-0004-9159-9051},
S.~P.~Wen$^{1}$\BESIIIorcid{0000-0003-3521-5338},
U.~Wiedner$^{3}$\BESIIIorcid{0000-0002-9002-6583},
G.~Wilkinson$^{75}$\BESIIIorcid{0000-0001-5255-0619},
M.~Wolke$^{81}$,
J.~F.~Wu$^{1,9}$\BESIIIorcid{0000-0002-3173-0802},
L.~H.~Wu$^{1}$\BESIIIorcid{0000-0001-8613-084X},
L.~J.~Wu$^{20}$\BESIIIorcid{0000-0002-3171-2436},
Lianjie~Wu$^{20}$\BESIIIorcid{0009-0008-8865-4629},
S.~G.~Wu$^{1,70}$\BESIIIorcid{0000-0002-3176-1748},
S.~M.~Wu$^{70}$\BESIIIorcid{0000-0002-8658-9789},
X.~W.~Wu$^{78}$\BESIIIorcid{0000-0002-6757-3108},
Y.~J.~Wu$^{34}$\BESIIIorcid{0009-0002-7738-7453},
Z.~Wu$^{1,64}$\BESIIIorcid{0000-0002-1796-8347},
L.~Xia$^{77,64}$\BESIIIorcid{0000-0001-9757-8172},
B.~H.~Xiang$^{1,70}$\BESIIIorcid{0009-0001-6156-1931},
D.~Xiao$^{42,k,l}$\BESIIIorcid{0000-0003-4319-1305},
G.~Y.~Xiao$^{46}$\BESIIIorcid{0009-0005-3803-9343},
H.~Xiao$^{78}$\BESIIIorcid{0000-0002-9258-2743},
Y.~L.~Xiao$^{12,g}$\BESIIIorcid{0009-0007-2825-3025},
Z.~J.~Xiao$^{45}$\BESIIIorcid{0000-0002-4879-209X},
C.~Xie$^{46}$\BESIIIorcid{0009-0002-1574-0063},
K.~J.~Xie$^{1,70}$\BESIIIorcid{0009-0003-3537-5005},
Y.~Xie$^{54}$\BESIIIorcid{0000-0002-0170-2798},
Y.~G.~Xie$^{1,64}$\BESIIIorcid{0000-0003-0365-4256},
Y.~H.~Xie$^{6}$\BESIIIorcid{0000-0001-5012-4069},
Z.~P.~Xie$^{77,64}$\BESIIIorcid{0009-0001-4042-1550},
T.~Y.~Xing$^{1,70}$\BESIIIorcid{0009-0006-7038-0143},
C.~J.~Xu$^{65}$\BESIIIorcid{0000-0001-5679-2009},
G.~F.~Xu$^{1}$\BESIIIorcid{0000-0002-8281-7828},
H.~Y.~Xu$^{2}$\BESIIIorcid{0009-0004-0193-4910},
M.~Xu$^{77,64}$\BESIIIorcid{0009-0001-8081-2716},
Q.~J.~Xu$^{17}$\BESIIIorcid{0009-0005-8152-7932},
Q.~N.~Xu$^{32}$\BESIIIorcid{0000-0001-9893-8766},
T.~D.~Xu$^{78}$\BESIIIorcid{0009-0005-5343-1984},
X.~P.~Xu$^{60}$\BESIIIorcid{0000-0001-5096-1182},
Y.~Xu$^{12,g}$\BESIIIorcid{0009-0008-8011-2788},
Y.~C.~Xu$^{83}$\BESIIIorcid{0000-0001-7412-9606},
Z.~S.~Xu$^{70}$\BESIIIorcid{0000-0002-2511-4675},
F.~Yan$^{24}$\BESIIIorcid{0000-0002-7930-0449},
L.~Yan$^{12,g}$\BESIIIorcid{0000-0001-5930-4453},
W.~B.~Yan$^{77,64}$\BESIIIorcid{0000-0003-0713-0871},
W.~C.~Yan$^{86}$\BESIIIorcid{0000-0001-6721-9435},
W.~H.~Yan$^{6}$\BESIIIorcid{0009-0001-8001-6146},
W.~P.~Yan$^{20}$\BESIIIorcid{0009-0003-0397-3326},
X.~Q.~Yan$^{12,g}$\BESIIIorcid{0009-0002-1018-1995},
X.~Q.~Yan$^{12,g}$\BESIIIorcid{0009-0002-1018-1995},
Y.~Y.~Yan$^{66}$\BESIIIorcid{0000-0003-3584-496X},
H.~J.~Yang$^{56,f}$\BESIIIorcid{0000-0001-7367-1380},
H.~L.~Yang$^{38}$\BESIIIorcid{0009-0009-3039-8463},
H.~X.~Yang$^{1}$\BESIIIorcid{0000-0001-7549-7531},
J.~H.~Yang$^{46}$\BESIIIorcid{0009-0005-1571-3884},
R.~J.~Yang$^{20}$\BESIIIorcid{0009-0007-4468-7472},
Y.~Yang$^{12,g}$\BESIIIorcid{0009-0003-6793-5468},
Y.~H.~Yang$^{46}$\BESIIIorcid{0000-0002-8917-2620},
Y.~Q.~Yang$^{10}$\BESIIIorcid{0009-0005-1876-4126},
Y.~Z.~Yang$^{20}$\BESIIIorcid{0009-0001-6192-9329},
Z.~P.~Yao$^{54}$\BESIIIorcid{0009-0002-7340-7541},
M.~Ye$^{1,64}$\BESIIIorcid{0000-0002-9437-1405},
M.~H.~Ye$^{9,\dagger}$\BESIIIorcid{0000-0002-3496-0507},
Z.~J.~Ye$^{61,j}$\BESIIIorcid{0009-0003-0269-718X},
Junhao~Yin$^{47}$\BESIIIorcid{0000-0002-1479-9349},
Z.~Y.~You$^{65}$\BESIIIorcid{0000-0001-8324-3291},
B.~X.~Yu$^{1,64,70}$\BESIIIorcid{0000-0002-8331-0113},
C.~X.~Yu$^{47}$\BESIIIorcid{0000-0002-8919-2197},
G.~Yu$^{13}$\BESIIIorcid{0000-0003-1987-9409},
J.~S.~Yu$^{27,i}$\BESIIIorcid{0000-0003-1230-3300},
L.~W.~Yu$^{12,g}$\BESIIIorcid{0009-0008-0188-8263},
T.~Yu$^{78}$\BESIIIorcid{0000-0002-2566-3543},
X.~D.~Yu$^{50,h}$\BESIIIorcid{0009-0005-7617-7069},
Y.~C.~Yu$^{86}$\BESIIIorcid{0009-0000-2408-1595},
Y.~C.~Yu$^{42}$\BESIIIorcid{0009-0003-8469-2226},
C.~Z.~Yuan$^{1,70}$\BESIIIorcid{0000-0002-1652-6686},
H.~Yuan$^{1,70}$\BESIIIorcid{0009-0004-2685-8539},
J.~Yuan$^{38}$\BESIIIorcid{0009-0005-0799-1630},
J.~Yuan$^{49}$\BESIIIorcid{0009-0007-4538-5759},
L.~Yuan$^{2}$\BESIIIorcid{0000-0002-6719-5397},
M.~K.~Yuan$^{12,g}$\BESIIIorcid{0000-0003-1539-3858},
S.~H.~Yuan$^{78}$\BESIIIorcid{0009-0009-6977-3769},
Y.~Yuan$^{1,70}$\BESIIIorcid{0000-0002-3414-9212},
C.~X.~Yue$^{43}$\BESIIIorcid{0000-0001-6783-7647},
Ying~Yue$^{20}$\BESIIIorcid{0009-0002-1847-2260},
A.~A.~Zafar$^{79}$\BESIIIorcid{0009-0002-4344-1415},
F.~R.~Zeng$^{54}$\BESIIIorcid{0009-0006-7104-7393},
S.~H.~Zeng$^{69}$\BESIIIorcid{0000-0001-6106-7741},
X.~Zeng$^{12,g}$\BESIIIorcid{0000-0001-9701-3964},
Yujie~Zeng$^{65}$\BESIIIorcid{0009-0004-1932-6614},
Y.~J.~Zeng$^{1,70}$\BESIIIorcid{0009-0005-3279-0304},
Y.~C.~Zhai$^{54}$\BESIIIorcid{0009-0000-6572-4972},
Y.~H.~Zhan$^{65}$\BESIIIorcid{0009-0006-1368-1951},
Shunan~Zhang$^{75}$\BESIIIorcid{0000-0002-2385-0767},
B.~L.~Zhang$^{1,70}$\BESIIIorcid{0009-0009-4236-6231},
B.~X.~Zhang$^{1,\dagger}$\BESIIIorcid{0000-0002-0331-1408},
D.~H.~Zhang$^{47}$\BESIIIorcid{0009-0009-9084-2423},
G.~Y.~Zhang$^{20}$\BESIIIorcid{0000-0002-6431-8638},
G.~Y.~Zhang$^{1,70}$\BESIIIorcid{0009-0004-3574-1842},
H.~Zhang$^{77,64}$\BESIIIorcid{0009-0000-9245-3231},
H.~Zhang$^{86}$\BESIIIorcid{0009-0007-7049-7410},
H.~C.~Zhang$^{1,64,70}$\BESIIIorcid{0009-0009-3882-878X},
H.~H.~Zhang$^{65}$\BESIIIorcid{0009-0008-7393-0379},
H.~Q.~Zhang$^{1,64,70}$\BESIIIorcid{0000-0001-8843-5209},
H.~R.~Zhang$^{77,64}$\BESIIIorcid{0009-0004-8730-6797},
H.~Y.~Zhang$^{1,64}$\BESIIIorcid{0000-0002-8333-9231},
J.~Zhang$^{65}$\BESIIIorcid{0000-0002-7752-8538},
J.~J.~Zhang$^{57}$\BESIIIorcid{0009-0005-7841-2288},
J.~L.~Zhang$^{21}$\BESIIIorcid{0000-0001-8592-2335},
J.~Q.~Zhang$^{45}$\BESIIIorcid{0000-0003-3314-2534},
J.~S.~Zhang$^{12,g}$\BESIIIorcid{0009-0007-2607-3178},
J.~W.~Zhang$^{1,64,70}$\BESIIIorcid{0000-0001-7794-7014},
J.~X.~Zhang$^{42,k,l}$\BESIIIorcid{0000-0002-9567-7094},
J.~Y.~Zhang$^{1}$\BESIIIorcid{0000-0002-0533-4371},
J.~Z.~Zhang$^{1,70}$\BESIIIorcid{0000-0001-6535-0659},
Jianyu~Zhang$^{70}$\BESIIIorcid{0000-0001-6010-8556},
L.~M.~Zhang$^{67}$\BESIIIorcid{0000-0003-2279-8837},
Lei~Zhang$^{46}$\BESIIIorcid{0000-0002-9336-9338},
N.~Zhang$^{38}$\BESIIIorcid{0009-0008-2807-3398},
P.~Zhang$^{1,9}$\BESIIIorcid{0000-0002-9177-6108},
Q.~Zhang$^{20}$\BESIIIorcid{0009-0005-7906-051X},
Q.~Y.~Zhang$^{38}$\BESIIIorcid{0009-0009-0048-8951},
R.~Y.~Zhang$^{42,k,l}$\BESIIIorcid{0000-0003-4099-7901},
S.~H.~Zhang$^{1,70}$\BESIIIorcid{0009-0009-3608-0624},
Shulei~Zhang$^{27,i}$\BESIIIorcid{0000-0002-9794-4088},
X.~M.~Zhang$^{1}$\BESIIIorcid{0000-0002-3604-2195},
X.~Y.~Zhang$^{54}$\BESIIIorcid{0000-0003-4341-1603},
Y.~Zhang$^{1}$\BESIIIorcid{0000-0003-3310-6728},
Y.~Zhang$^{78}$\BESIIIorcid{0000-0001-9956-4890},
Y.~T.~Zhang$^{86}$\BESIIIorcid{0000-0003-3780-6676},
Y.~H.~Zhang$^{1,64}$\BESIIIorcid{0000-0002-0893-2449},
Y.~P.~Zhang$^{77,64}$\BESIIIorcid{0009-0003-4638-9031},
Z.~D.~Zhang$^{1}$\BESIIIorcid{0000-0002-6542-052X},
Z.~H.~Zhang$^{1}$\BESIIIorcid{0009-0006-2313-5743},
Z.~L.~Zhang$^{38}$\BESIIIorcid{0009-0004-4305-7370},
Z.~L.~Zhang$^{60}$\BESIIIorcid{0009-0008-5731-3047},
Z.~X.~Zhang$^{20}$\BESIIIorcid{0009-0002-3134-4669},
Z.~Y.~Zhang$^{82}$\BESIIIorcid{0000-0002-5942-0355},
Z.~Y.~Zhang$^{47}$\BESIIIorcid{0009-0009-7477-5232},
Z.~Y.~Zhang$^{49}$\BESIIIorcid{0009-0004-5140-2111},
Zh.~Zh.~Zhang$^{20}$\BESIIIorcid{0009-0003-1283-6008},
G.~Zhao$^{1}$\BESIIIorcid{0000-0003-0234-3536},
J.~Y.~Zhao$^{1,70}$\BESIIIorcid{0000-0002-2028-7286},
J.~Z.~Zhao$^{1,64}$\BESIIIorcid{0000-0001-8365-7726},
L.~Zhao$^{1}$\BESIIIorcid{0000-0002-7152-1466},
L.~Zhao$^{77,64}$\BESIIIorcid{0000-0002-5421-6101},
M.~G.~Zhao$^{47}$\BESIIIorcid{0000-0001-8785-6941},
S.~J.~Zhao$^{86}$\BESIIIorcid{0000-0002-0160-9948},
Y.~B.~Zhao$^{1,64}$\BESIIIorcid{0000-0003-3954-3195},
Y.~L.~Zhao$^{60}$\BESIIIorcid{0009-0004-6038-201X},
Y.~P.~Zhao$^{49}$\BESIIIorcid{0009-0009-4363-3207},
Y.~X.~Zhao$^{34,70}$\BESIIIorcid{0000-0001-8684-9766},
Z.~G.~Zhao$^{77,64}$\BESIIIorcid{0000-0001-6758-3974},
A.~Zhemchugov$^{40,b}$\BESIIIorcid{0000-0002-3360-4965},
B.~Zheng$^{78}$\BESIIIorcid{0000-0002-6544-429X},
B.~M.~Zheng$^{38}$\BESIIIorcid{0009-0009-1601-4734},
J.~P.~Zheng$^{1,64}$\BESIIIorcid{0000-0003-4308-3742},
W.~J.~Zheng$^{1,70}$\BESIIIorcid{0009-0003-5182-5176},
X.~R.~Zheng$^{20}$\BESIIIorcid{0009-0007-7002-7750},
Y.~H.~Zheng$^{70,o}$\BESIIIorcid{0000-0003-0322-9858},
B.~Zhong$^{45}$\BESIIIorcid{0000-0002-3474-8848},
C.~Zhong$^{20}$\BESIIIorcid{0009-0008-1207-9357},
H.~Zhou$^{39,54,n}$\BESIIIorcid{0000-0003-2060-0436},
J.~Q.~Zhou$^{38}$\BESIIIorcid{0009-0003-7889-3451},
S.~Zhou$^{6}$\BESIIIorcid{0009-0006-8729-3927},
X.~Zhou$^{82}$\BESIIIorcid{0000-0002-6908-683X},
X.~K.~Zhou$^{6}$\BESIIIorcid{0009-0005-9485-9477},
X.~R.~Zhou$^{77,64}$\BESIIIorcid{0000-0002-7671-7644},
X.~Y.~Zhou$^{43}$\BESIIIorcid{0000-0002-0299-4657},
Y.~X.~Zhou$^{83}$\BESIIIorcid{0000-0003-2035-3391},
Y.~Z.~Zhou$^{12,g}$\BESIIIorcid{0000-0001-8500-9941},
A.~N.~Zhu$^{70}$\BESIIIorcid{0000-0003-4050-5700},
J.~Zhu$^{47}$\BESIIIorcid{0009-0000-7562-3665},
K.~Zhu$^{1}$\BESIIIorcid{0000-0002-4365-8043},
K.~J.~Zhu$^{1,64,70}$\BESIIIorcid{0000-0002-5473-235X},
K.~S.~Zhu$^{12,g}$\BESIIIorcid{0000-0003-3413-8385},
L.~X.~Zhu$^{70}$\BESIIIorcid{0000-0003-0609-6456},
Lin~Zhu$^{20}$\BESIIIorcid{0009-0007-1127-5818},
S.~H.~Zhu$^{76}$\BESIIIorcid{0000-0001-9731-4708},
T.~J.~Zhu$^{12,g}$\BESIIIorcid{0009-0000-1863-7024},
W.~D.~Zhu$^{12,g}$\BESIIIorcid{0009-0007-4406-1533},
W.~J.~Zhu$^{1}$\BESIIIorcid{0000-0003-2618-0436},
W.~Z.~Zhu$^{20}$\BESIIIorcid{0009-0006-8147-6423},
Y.~C.~Zhu$^{77,64}$\BESIIIorcid{0000-0002-7306-1053},
Z.~A.~Zhu$^{1,70}$\BESIIIorcid{0000-0002-6229-5567},
X.~Y.~Zhuang$^{47}$\BESIIIorcid{0009-0004-8990-7895},
J.~H.~Zou$^{1}$\BESIIIorcid{0000-0003-3581-2829}
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
$^{4}$ Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ Central South University, Changsha 410083, People's Republic of China\\
$^{8}$ Chengdu University of Technology, Chengdu 610059, People's Republic of China\\
$^{9}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{10}$ China University of Geosciences, Wuhan 430074, People's Republic of China\\
$^{11}$ Chung-Ang University, Seoul, 06974, Republic of Korea\\
$^{12}$ Fudan University, Shanghai 200433, People's Republic of China\\
$^{13}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{14}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{15}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{16}$ Guangxi University of Science and Technology, Liuzhou 545006, People's Republic of China\\
$^{17}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{18}$ Hebei University, Baoding 071002, People's Republic of China\\
$^{19}$ Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{20}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{21}$ Henan University, Kaifeng 475004, People's Republic of China\\
$^{22}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{23}$ Henan University of Technology, Zhengzhou 450001, People's Republic of China\\
$^{24}$ Hengyang Normal University, Hengyang 421001, People's Republic of China\\
$^{25}$ Huangshan College, Huangshan 245000, People's Republic of China\\
$^{26}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{27}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{28}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{29}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{30}$ INFN Laboratori Nazionali di Frascati, (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN Sezione di Perugia, I-06100, Perugia, Italy; (C)University of Perugia, I-06100, Perugia, Italy\\
$^{31}$ INFN Sezione di Ferrara, (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
$^{32}$ Inner Mongolia University, Hohhot 010021, People's Republic of China\\
$^{33}$ Institute of Business Administration, Karachi,\\
$^{34}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{35}$ Institute of Physics and Technology, Mongolian Academy of Sciences, Peace Avenue 54B, Ulaanbaatar 13330, Mongolia\\
$^{36}$ Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Casilla 7D, Arica 1000000, Chile\\
$^{37}$ Jiangsu Ocean University, Lianyungang 222000, People's Republic of China\\
$^{38}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{39}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{40}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{41}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{42}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{43}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{44}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{45}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{46}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{47}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{48}$ National Centre for Nuclear Research, Warsaw 02-093, Poland\\
$^{49}$ North China Electric Power University, Beijing 102206, People's Republic of China\\
$^{50}$ Peking University, Beijing 100871, People's Republic of China\\
$^{51}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{52}$ Renmin University of China, Beijing 100872, People's Republic of China\\
$^{53}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{54}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{55}$ Shandong University of Technology, Zibo 255000, People's Republic of China\\
$^{56}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
$^{57}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{58}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{59}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{60}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{61}$ South China Normal University, Guangzhou 510006, People's Republic of China\\
$^{62}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{63}$ Southwest University of Science and Technology, Mianyang 621010, People's Republic of China\\
$^{64}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{65}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{66}$ Suranaree University of Technology, University Avenue 111, Nakhon Ratchasima 30000, Thailand\\
$^{67}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{68}$ Turkish Accelerator Center Particle Factory Group, (A)Istinye University, 34010, Istanbul, Turkey; (B)Near East University, Nicosia, North Cyprus, 99138, Mersin 10, Turkey\\
$^{69}$ University of Bristol, H H Wills Physics Laboratory, Tyndall Avenue, Bristol, BS8 1TL, UK\\
$^{70}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{71}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{72}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{73}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{74}$ University of Muenster, Wilhelm-Klemm-Strasse 9, 48149 Muenster, Germany\\
$^{75}$ University of Oxford, Keble Road, Oxford OX13RH, United Kingdom\\
$^{76}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{77}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{78}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{79}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{80}$ University of Turin and INFN, (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{81}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{82}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{83}$ Yantai University, Yantai 264005, People's Republic of China\\
$^{84}$ Yunnan University, Kunming 650500, People's Republic of China\\
$^{85}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{86}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\

\vspace{0.2cm}
$^{\dagger}$ Deceased\\
$^{a}$ Also at Bogazici University, 34342 Istanbul, Turkey\\
$^{b}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{c}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{d}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{e}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{f}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{g}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{h}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{i}$ Also at School of Physics and Electronics, Hunan University, Changsha 410082, China\\
$^{j}$ Also at Guangdong Provincial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou 510006, China\\
$^{k}$ Also at MOE Frontiers Science Center for Rare Isotopes, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{l}$ Also at Lanzhou Center for Theoretical Physics, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{m}$ Also at Ecole Polytechnique Federale de Lausanne (EPFL), CH-1015 Lausanne, Switzerland\\
$^{n}$ Also at Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{o}$ Also at Hangzhou Institute for Advanced Study, University of Chinese Academy of Sciences, Hangzhou 310024, China\\
$^{p}$ Currently at Silesian University in Katowice, Chorzow, 41-500, Poland\\
$^{q}$ Also at Applied Nuclear Technology in Geosciences Key Laboratory of Sichuan Province, Chengdu University of Technology, Chengdu 610059, People's Republic of China\\

}
%% ends here %%

